Revealing User Familiarity Bias in Task-Oriented Dialogue via Interactive Evaluation

Most task-oriented dialogue (TOD) benchmarks assume users that know exactly how to use the system by constraining the user behaviors within the system's capabilities via strict user goals, namely "user familiarity" bias. This data bias deepens when it combines with data-driven TOD systems, as it is impossible to fathom the effect of it with existing static evaluations. Hence, we conduct an interactive user study to unveil how vulnerable TOD systems are against realistic scenarios. In particular, we compare users with 1) detailed goal instructions that conform to the system boundaries (closed-goal) and 2) vague goal instructions that are often unsupported but realistic (open-goal). Our study reveals that conversations in open-goal settings lead to catastrophic failures of the system, in which 92% of the dialogues had significant issues. Moreover, we conduct a thorough analysis to identify distinctive features between the two settings through error annotation. From this, we discover a novel "pretending" behavior, in which the system pretends to handle the user requests even though they are beyond the system's capabilities. We discuss its characteristics and toxicity while showing recent large language models can also suffer from this behavior.

==> figure/overview.tex <==
\begin{figure*}[h!]
    \centering
    \includegraphics[width=\textwidth]{assets/fig_overview.pdf}
    \caption{An illustration of exceptional requests in task-oriented dialogue system. Exceptional requests are not covered by the parametric system and prepared exceptional knowledge.} 
    \label{fig:overview}
\end{figure*}

==> figure/plugin.tex <==
\begin{figure*}[h!]
    \centering
    \includegraphics[width=0.7\textwidth]{assets/fig_plugin.pdf}
    \caption{An example of ChatGPT with plugins captured from \url{https://openai.com/blog/chatgpt-plugins}. User in this example shows high familiarity of the service, while real users are expected to behave with low familiarity. This tendency will increase in the scenario of multi-plugin situations because only a few users are familiar with capacities of all services.}
    \label{fig:plugin}
\end{figure*}

